POSEFusion: Pose-guided Selective Fusion for Single-view Human Volumetric Capture

We propose POse-guided SElective Fusion (POSEFusion), a single-view human volumetric capture method that leverages tracking-based methods and tracking-free inference to achieve high-fidelity and dynamic 3D reconstruction. By contributing a novel reconstruction framework which contains pose-guided keyframe selection and robust implicit surface fusion, our method fully utilizes the advantages of both tracking-based methods and tracking-free inference methods, and finally enables the high-fidelity reconstruction of dynamic surface details even in the invisible regions. We formulate the keyframe selection as a dynamic programming problem to guarantee the temporal continuity of the reconstructed sequence. Moreover, the novel robust implicit surface fusion involves an adaptive blending weight to preserve high-fidelity surface details and an automatic collision handling method to deal with the potential self-collisions. Overall, our method enables high-fidelity and dynamic capture in both visible and invisible regions from a single RGBD camera, and the results and experiments show that our method outperforms state-of-the-art methods.

==> sections/1_intro_old.tex <==
\section{Introduction}
Human volumetric capture, due to their potential value in holographic communication, online education, game and movie production, has been a popular topic in computer vision and graphics for decades. Multi-view camera array methods \cite{bradley2008markerless, gall2009motion, liu2009point, brox2009combined, liu2011markerless, ye2012performance, mustafa2015general, dou2016fusion4d, pons2017clothcap, leroy2017multi} are able to achieve high-fidelity human volumetric capture using multiple RGB or depth sensors, but suffer from sophisticated equipment or run-time inefficiency, which limit their application deployment. In contrast, single-view human volumetric capture \cite{li2009robust, zollhofer2014real, guo2015robust, newcombe2015dynamicfusion, yu2018doublefusion, habermann2019livecap, saito2019pifu, saito2020pifuhd, habermann2020deepcap, li2020monocular, su2020robustfusion} has attracted more and more attention for its convenient setups.

Current methods for single-view human volumetric capture can be roughly classified into two categories: tracking-based methods and tracking-free ones. Tracking-based methods utilize a pre-scanned template \cite{li2009robust, guo2015robust, habermann2019livecap, habermann2020deepcap} or continuously fused mesh \cite{newcombe2015dynamicfusion, yu2018doublefusion, su2020robustfusion} as the reference model, and solve or infer the deformation of the reference model parameterized by embedded skeletons \cite{ye2014real, bogo2015detailed, xu2018monoperfcap}, node graph \cite{li2009robust, newcombe2015dynamicfusion} or both of them \cite{yu2017BodyFusion, yu2018doublefusion, habermann2019livecap, habermann2020deepcap}.
%Some previous works in tracking-based methods utilize a person-specific template with embedded skeletons \cite{gall2009motion, liu2011markerless, ye2012performance, ye2014real, habermann2019livecap} or node graph \cite{li2009robust, guo2015robust, zollhofer2014real, habermann2019livecap} and deform it to track each RGB(D) input. DynamicFusion \cite{newcombe2015dynamicfusion} pioneered the direction of free-from dynamic reconstruction by replacing the specific template with a continuously fused model. Focusing on human performance capture, DoubleFusion \cite{yu2018doublefusion} combined the parametric SMPL model \cite{loper2015smpl} for more robust body tracking. 
In these tracking-based methods, previous observations are integrated into the current frame after calculating the deformations across frames, thus plausible geometric details are preserved in the invisible regions. In addition, the reconstructed models are temporally continuous thanks to frame-by-frame tracking. However, none of their deformation representations, neither skeletons nor node graph, is able to handle topological changes (Fig.~) or describe extremely non-rigid deformation (Fig.~), which is an essential drawback of tracking-based methods.

On the other end of the spectrum, tracking-free methods, main methods for single-frame inference\cite{varol2018bodynet, natsume2019siclope, gabeur2019moulding, smith2019facsimile, zhu2019detailed, alldieck2019tex2shape, zheng2019deephuman, saito2019pifu}, focus on geometric and/or texture recovery from a single RGB(D) image. By learning from a large amount of 3D human data, these methods demonstrate promising human reconstruction with high-resolution details in visible regions and plausible shape in invisible areas\cite{saito2019pifu, saito2020pifuhd}. As the reconstruction for the current frame is independent from previous ones, these methods can easily handle topological changes. However, because of the dependence on the variety of the training dataset, their results may deteriorate in the cases of challenging human motions and/or self-occluded poses. Even though geometric details can be directly reconstructed in the visible regions, the invisible regions are usually oversmooth for the lack of observations. What's worse, tracking-free methods are incapable of generating temporally continuous results when applied on video inputs. 
% Moreover, since these methods focus on recovery from a single image, the reconstructed models from a single-view video also lack temporal smoothness.

%From the perspective of the dependence on a reference model, single-view human volumetric capture can be classified into deformation-based and deformation-free methods. Deformation-based methods utilize a pre-scanned template \cite{li2009robust, guo2015robust, habermann2019livecap, habermann2020deepcap} or continuously fused mesh \cite{newcombe2015dynamicfusion, yu2018doublefusion} as the reference model, and solve or infer the deformation of the reference model parameterized by embedded skeletons \cite{ye2014real, bogo2015detailed, xu2018monoperfcap}, node graph \cite{li2009robust, newcombe2015dynamicfusion} or both of them \cite{yu2017BodyFusion, yu2018doublefusion, habermann2019livecap, habermann2020deepcap}. These methods can reconstruct temporally continuous models from a single-view RGB(D) video. However, neither skeletal nor node-graph-based parameterization cannot describe extremely non-rigid deformation (Fig.~) and handle topological change (Fig.~), which are natural and essential drawbacks of deformation-based methods. On the other hand, deformation-free methods \cite{zheng2019deephuman, saito2019pifu, saito2020pifuhd, li2020monocular} usually focus on single-frame reconstruction by learning from a large amount of 3D models. Without the dependence on the deformation of a reference model, these methods can handle topological change based on the current observation, but lack temporal continuity.

%By reviewing the advantages and the drawbacks of deformation-based and deformation-free methods, we notice that these two types are naturally complemental as shown in Tab.~\ref{tab: comparison of methods}. We therefore propose Implicit Surface Fusion (ISF) to resolve all the drawbacks and maintain all the advantages mentioned above. However, combining these two types of methods is non-trivial. Our observation is that deformation-free methods (\cite{saito2019pifu, saito2020pifuhd}) can infer high-fidelity details in visible regions and plausible geometry in invisible regions, so solving an accurate and fine-level deformation of a fused or pre-scanned template as in deformation-based methods is not necessary. Thus a coarse-level skeletal motion is enough to represent the body motion among frames, in our approach, we utilize SMPL \cite{loper2015smpl} to represent the body motion conveniently and robustly. Our another observation is that deformation-based methods \cite{li2009robust, newcombe2015dynamicfusion} can reserve geometric details in invisible regions by integrating previous observations. We therefore propose to integrate inferred occupancy values by a deformation-free method into the current frame to not only guarantee high-fidelity appearances and deformations in visible regions but also reserve geometric details provided by previous observations in invisible regions. The continuous distribution of occupancy values and the designed robust blending weight also guarantee the smooth transition from visible to invisible regions. Based on these two observations, our method do not rely on a fused or pre-scanned reference model and can handle topological change well. Moreover, our method not only maintains temporal continuity, which is the inherent advantage of tracking-based methods, but is also able to handle challenging poses or self-occluded input because the geometry in invisible regions depends on previous visible observations rather than the current low-confident inference.

%On the other end of the spectrum, single-view human volumetric capture can be also classified into data-driven and fusion-based methods according to the generation of invisible regions. Data-driven methods \cite{zheng2019deephuman, saito2019pifu, zhi2020texmesh} infer a plausible surface in invisible regions but lack geometric details because the network trends to learn a mean level set. Although fusion-based methods \cite{newcombe2015dynamicfusion, li2009robust, yu2018doublefusion} integrate the previous observations into the current frame to generate a complete model, fusing all the previous input without adaptive selection makes the invisible details immutable during the whole capture. To this end, we propose a pose-dependent keyframe selection scheme to select appropriate keyframes by pose similarity and visibility rather than integrate all the previous frames while avoiding temporally discontinuity of invisible details.

\begin{table*}[t]
    \footnotesize
    \centering
    \begin{tabular}{ccccccc}
      \hline
      \multicolumn{2}{c}{Methods}                                                                      & \begin{tabular}[c]{@{}c@{}}Topological\\ Change\end{tabular} & \begin{tabular}[c]{@{}c@{}}Natural\\ Deformation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Details in\\ Invisible Regions\end{tabular}    & \begin{tabular}[c]{@{}c@{}}Temporal\\ Continuity\end{tabular} & Texture\\
      \hline
      \textbf{Tracking-based} & DoubleFusion \cite{yu2018doublefusion} & \wrong & \wrong & {\correct (Static)} & \correct & None\\
      \cline{2-7}
      & RobustFusion \cite{su2020robustfusion} & \wrong & \wrong & {\correct (Static)} & \correct & {\correct (Low-quality)}\\
      \hline
      \textbf{Single-frame Inference} & PIFu \cite{saito2019pifu}/PIFuHD \cite{saito2020pifuhd} & \correct & \correct & \wrong & \wrong & {\correct (Low-quality)}\\
      \hline
      \textbf{Others} & TexMesh \cite{zhi2020texmesh} & \wrong & \wrong & \correct (Low-quality) & \correct & \correct (Static) \\
      \hline
      \multicolumn{2}{c}{\textbf{Ours}} & \correct & \correct & \begin{tabular}[c]{@{}c@{}}\ding{51}\\ (Dynamic, High-quality)\end{tabular} & \correct & \begin{tabular}[c]{@{}c@{}}\ding{51}\\ (Dynamic, High-quality)\end{tabular}\\
      \hline
    \end{tabular}
    \caption{Comparison of our method with other works. Our method inherits all the advantages of tracking-based methods and tracking-free inference while avoiding all the drawbacks. Moreover, our method can reconstruct dynamic pose-dependent geometric details and high-quality texture.}
    \label{tab: comparison of methods}
\end{table*}


% Zerong's revision: 
By reviewing the advantages and the drawbacks of these two types of methods, it is easy to notice that tracking-based methods and tracking-free inference are naturally complementary as shown in Tab.~\ref{tab: comparison of methods}.
As such, one might consider combining the best of both worlds. 
A potential pipeline is firstly inferring the models for all video frames individually and then fusing all the models to recover the invisible shapes for each frame. 
However, it won't lead to satisfactory results due to the challenges of: a) human body tracking of the fast motion b) over-smooth reconstruction when fusing the whole sequences, c) erroneous inference results in occluded regions, and d) possible collision and separation of body parts resulting from body motions. 
To overcome these challenges, we propose Implicit Surface Fusion (ISF), a pipeline that is able to reconstruct complete, dynamic and high-fidelity 3D human models from a single-view RGBD sequence. 
[TODO: organize contribution according to the challenges mentioned above] 
Our observation is that given the current input, single-frame inference can reconstruct high-fidelity visible details and plausible invisible geometry, so solving an accurate and fine-level deformation of a fused or pre-scanned template as in deformation-based methods is not necessary. Thus a coarse-level skeletal motion is enough to represent the body motion among frames. In our approach, we utilize SMPL \cite{loper2015smpl} to represent the body motion conveniently and robustly. Our another observation is that deformation-based methods \cite{li2009robust, newcombe2015dynamicfusion} can reserve geometric details in invisible regions by integrating previous observations. We therefore propose to integrate inferred occupancy values by single-frame inference into the current frame to not only guarantee high-fidelity appearances and deformations in the visible region but also reserve geometric details provided by previous observations in the invisible region. The continuous distribution of occupancy values and the designed robust blending weight also guarantee the smooth transition from visible to invisible regions. Based on these two observations, our method do not rely on a fused or pre-scanned model and can handle topological change well. Moreover, our method not only maintains temporal continuity, which is the inherent advantage of tracking-based methods, but is also able to handle challenging poses or self-occluded input because the geometry in invisible regions depends on previous visible observations rather than the current low-confident inference.

% old version
% By reviewing the advantages and the drawbacks of these two types of methods, it is easy to notice that tracking-based methods and tracking-free inference are naturally complementary as shown in Tab.~\ref{tab: comparison of methods}. We therefore propose Implicit Surface Fusion (ISF) to resolve all the drawbacks and maintain all the advantages mentioned above. However, combining these two types of methods is non-trivial. Our observation is that given the current input, single-frame inference can reconstruct high-fidelity visible details and plausible invisible geometry, so solving an accurate and fine-level deformation of a fused or pre-scanned template as in deformation-based methods is not necessary. Thus a coarse-level skeletal motion is enough to represent the body motion among frames, in our approach, we utilize SMPL \cite{loper2015smpl} to represent the body motion conveniently and robustly. Our another observation is that deformation-based methods \cite{li2009robust, newcombe2015dynamicfusion} can reserve geometric details in invisible regions by integrating previous observations. We therefore propose to integrate inferred occupancy values by single-frame inference into the current frame to not only guarantee high-fidelity appearances and deformations in the visible region but also reserve geometric details provided by previous observations in the invisible region. The continuous distribution of occupancy values and the designed robust blending weight also guarantee the smooth transition from visible to invisible regions. Based on these two observations, our method do not rely on a fused or pre-scanned model and can handle topological change well. Moreover, our method not only maintains temporal continuity, which is the inherent advantage of deformation-based methods, but is also able to handle challenging poses or self-occluded input because the geometry in invisible regions depends on previous visible observations rather than the current low-confident inference.


% old version
%By reviewing the advantages and drawbacks of these two types of methods, we notice that tracking-based methods and learning-based methods can complement each other fortunately as shown in Tab.~\ref{tab: comparison of methods}. We therefore propose Implicit Surface Fusion (ISF) to resolve all the drawbacks and maintain all the advantages mentioned above. However, combining these two types of methods is non-trivial.  First, we need to solve the body motion between frames. To conveniently and robustly represent the forward and backward body motion, we track each depth input by solving the skeletal motion of SMPL \cite{loper2015smpl}. But skeleton-level motion cannot describe non-rigid deformation on body surface, e.g., clothing wrinkles. Our observation is that learning-based methods (\cite{saito2019pifu, saito2020pifuhd}) can infer high-fidelity details in the visible region and plausible geometry in the invisible region, so solving an accurate and fine-level deformation of a fused or pre-scanned template is not necessary. However, the invisible region is usually oversmooth because the neural network trends to learn a mean level set. Inspired by tracking-based methods \cite{newcombe2015dynamicfusion}, we propose to integrate inferred occupancy values by PIFu \cite{saito2019pifu} into the current frame to not only guarantee high-fidelity appearances and deformations in the visible region but also reserve geometric details provided by previous observations in the invisible region. Thanks to no need to deform a specific or fused template to track input, our method can handle topological change in visible regions well. Moreover, our method not only maintains temporal continuity, the inherent advantage of tracking-based methods, but also can handle challenging poses or self-occluded input because of the SMPL motion prior.

Though tracking-based methods \cite{newcombe2015dynamicfusion, li2009robust} can integrate details into the invisible region, fusing all the previous input without adaptive selection makes the invisible details immutable during the whole capture. Our insight is that the SMPL model \cite{loper2015smpl} across the whole sequence contributes to quantify pose and visibility conveniently. To this end, we propose a pose-dependent keyframe selection scheme and formulate it into a dynamic programming problem to select appropriate keyframes by pose similarity and visibility complemtarity rather than integrate all the previous frames while avoiding temporally discontinuity of invisible details.

% collision
Although the pipeline has been carefully designed, it still suffers from the collision problem. Consider two body parts are collided with each other in the current frame, it is confusing to decide which body part to drive each sampled point around the collided regions. Due to the tracking error and the difference between the real clothed body with SMPL model, the collided points may be warped to a wrong position and fetch wrong occupancy values. To this end, we propose a collision handling scheme, which aims to warp the reconstructed model without collision of an adjacent frame to the current frame, and consider this model into the final fusion.

In summary, by the good combination of tracking-based methods and tacking-free inference, Implicit Surface Fusion (ISF) leverages all the advantages of the two branches while avoiding all the drawbacks, and finally enables human volumetric capture with dynamic and fine details in both visible and invisible regions from a single RGBD camera.

The main technical contributions of ISF can be summarized as:
\begin{itemize}
% \setlength{\itemsep}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\parskip}{0pt}
	\item A new human volumetric capture pipeline that leverages tracking-based methods and single-frame inference, and achieves high-quality and dynamic reconstruction in both visible and invisible regions from a single RGBD camera.
	\item A new pose-guided keyframe selection scheme that considers both pose similarity and visibility and enables detailed and pose-guided reconstruction in the invisible region.
	\item A robust blending scheme ...
	\item A automatic collision handling scheme that considers an adjacent model without collision into the fusion procedure to reserve the adjacent details while avoiding collision artifacts.
\end{itemize}



==> sections/supp_single.tex <==
In this supplementary material, we mainly introduce our implementation details, the system performance, and additional experiments.
\section{Implementation Details}
\subsection{Initialization}
Given the tracked SMPL model \cite{loper2015smpl} in the current frame, we firstly allocate a 3D volume which contains the SMPL. For each voxel, we calculate the Euclidean distance between its center with SMPL, and select valid voxels (points) near the SMPL with a threshold of 8cm.

\subsection{Pose-guided Keyframe Selection}
\noindent\textbf{SMPL Remeshing} Due to the uneven distribution of vertices of the original SMPL \cite{loper2015smpl}, we remesh the original SMPL into an isotropic triangular template using \cite{jakob2015instant} as shown in Fig.~\ref{fig:smpl remeshing}. We then transfer the parameters (e.g., blending weights) in \cite{loper2015smpl} to the new template. Using the new template with uniform triangles, the visibility energy can be calculated without the negative impact of dense vertices in the face and hand regions as shown in Fig.~\ref{fig:smpl remeshing}(a). In our experiment, the new template contains 6839 vertices and 13690 faces. For simplicity, we also call the new template SMPL in the main paper and this supplementary material.

\noindent\textbf{Block Division by Visibility}
Though the formulated dynamic programming (DP) solution can provide a temporally continuous keyframe trail, this trail in the first iteration denoted as $\mathcal{T}^1$ may cross the diagonal region of the energy matrix $E$ (the red rectangle in Fig.~\ref{fig:block-wise refine}(a)), which indicates that in this region the selected keyframe $t_i$ is very close to the current $i$-th frame, i.e., the $i$-th and $t_i$-th frames have roughly the same visible region of the human body. In the second iteration, the DP generates another trail denoted as $\mathcal{T}^2$ as shown in Fig.~\ref{fig:block-wise refine}(b). It is obvious that for the red rectangle region $\mathcal{T}^2$ has more contribution for the visibility complementarity, however, $\mathcal{T}^2$ may be discontinuous with $\mathcal{T}^1$ on the boundary of the red rectangle. This will deteriorate the temporal continuity of the reconstructed details in invisible regions in this rectangle region.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures_supp/remesh_smpl.jpg}
    \caption{SMPL remeshing using \cite{jakob2015instant}. (a)(b) The wireframes of the original SMPL and the new template, respectively.}
    \label{fig:smpl remeshing}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/block_wise_refine.png}
    \caption{Illustration of the block division by the visibility energy. (a)(b) the keyframe trail on the energy matrix $E$ in the first and second iteration without block division, respectively, and in the red rectangle the selected keyframe in the first iteration is very close to the current frame; (c) the divided blocks by the visibility matrix $E_{\text{v}}$ of the first iteration.}
    \label{fig:block-wise refine}
    \vspace{-0.4cm}
\end{figure}

Our observation is that the red rectangle usually occurs when the visible region changes significantly, e.g., the performer turns from facing the camera to back facing it, which can be intuitively seen from the visibility matrix $E_{\text{v}}$ of the first iteration (the $(i,j)$-th element of $E_{\text{v}}$ is $1-E_{\text{visibility}}(\mathcal{K}_i,j)$) as shown in Fig.~\ref{fig:block-wise refine}(c). We therefore firstly divide the whole sequence as several blocks using  $E_{\text{v}}$ as shown in Fig.~\ref{fig:block-wise refine}(c). If the trail crosses two individual blocks, the red rectangle will be bounded, then we maintain a fixed-size FIFO (first-in-first-out) queue $\mathcal{Q}$ for the rectangle region and push the selected keyframes of previous frames into $\mathcal{Q}$. $\mathcal{Q}$ is considered as the keyframe set of the red rectangle region to guarantee the temporally smooth transition of the reconstructed invisible details. In our experiment, the threshold of block division is 0.3, and the size of $\mathcal{Q}$ is 10.

\subsection{Occupancy Inference}
Our occupancy inference network is based on PIFu \cite{saito2019pifu} which consists of a Stacked Hourglass network \cite{newell2016stacked} as the image encoder and a MLP with 258, 1024, 512, 256, 128, and 1 neurons in each layer. To fully utilize the depth information, we also encode the depth image and add a PSDF feature to MLP. The PSDF of a 3D point $\mathbf{x}$ is defined as
\begin{equation}
    PSDF(\mathbf{x}) = \left\{\begin{matrix}
\mathbf{x}_z-d & ,\mathbf{x}_z-d < 0\\ 
0 & ,\mathbf{x}_z-d \geq 0
\end{matrix}\right.,
\end{equation}
where $\mathbf{x}_z$ is the z-axis coordinate of $\mathbf{x}$, and $d$ is the depth value sampled at the projected location of $\mathbf{x}$ on the depth image.
We render a synthetic dataset (\url{https://web.twindom.com/}) to generate depth and color images as training data, and utilize 5000 images to train this network. When training, the batch size is 4, the learning rate is $1\times 10^{-3}$ and the number of epochs is 100.



\subsection{Collision Handling}
\noindent\textbf{Collision Detection} Based on the SMPL model, we first calculate the distance between every two vertices, and construct a symmetrical distance matrix $D\in\mathbb{R}^{N\times N}$ ($N$ is the vertex number), and $D_{ij}$ is the distance between the $i$-th and $j$-th vertices. For the current frame (the $t$-th frame) and one keyframe (the $k$-th frame), we calculate $D^{t}$ and $D^{k}$ respectively. And the collided vertices on the current SMPL are detected by the condition:
\begin{equation}
\begin{split}
\label{eq:collision condition}
    D_{ij}^t < \tau_1,\quad D_{ij}^k > \tau_2,
\end{split}
\end{equation}
which means that the $i$-th and $j$-th vertices collide with each other in the current frame. All the collided SMPL vertices are denoted as $\mathbf{V}_{\text{c}}$. The voxels corresponding to $\mathbf{V}_{\text{c}}$ are also detected. In our experiment, $\tau_1=0.02m$ and $\tau_2=0.05m$.

\noindent\textbf{Searching No-collision Frame} Starting from the current frame, we search for a no-collision frame both forward and backward. We calculate the proportion of SMPL vertices that belong to $\mathbf{V}_{\text{c}}$ but do not meet the collision condition (Eq.~\ref{eq:collision condition}) during searching each frame. If the proportion is less $30\%$, the no-collision frame is found. Then we deform the reconstructed model of the no-collision frame to the current frame, and integrate the deformed model into implicit surface fusion. In the fusion procedure, we first generate a 3D mask in the volume by the collision flag, and then perform 3D distance transform to generate a continuous weight volume for integrating the deformed model.

\subsection{Parameter Setting}
In the keyframe selection, we select $K=4$ keyframes for each frame. And in the first iteration, $\lambda_{\text{visibility}} = 1.5$, and $\lambda_{\text{visibility}} = 3.0$ in the subsequent iterations. In the adaptive blending weight, we set $\tau=0.02$ and $\sigma=100$.



\section{Performance}
We implement POSEFusion on one PC with one NVIDIA RTX 2080Ti, and the performance mainly depends on the number of keyframes. The time of processing one keyframe is almost 1.87 secs, which consists of 1.53 secs for deforming points and collision detection, 0.02 secs for loading images, 0.3 secs for occupancy inference, and 0.02 secs for blending occupancy values. In our experiment, we perform the pose-guided keyframe selection to select $K=4$ keyframes, and consider the current frame and the 3 frames around it as keyframes as well for denoising. So the keyframe number is $7$, and the time cost for reconstructing one frame is 13 secs. Moreover, we believe the runtime of this system could be further improved by TensorRT and other GPU toolkits.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures_supp/intermediate_results.jpg}
    \caption{Intermediate results during reconstruction of one frame. In each rectangle, from left to right are the reference color image, warped SMPL, dense reconstruction and color-encoded blending weights, respectively.}
    \label{fig:intermediate results}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures_supp/eval_greedy.png}
    \caption{Quantitative comparison against the greedy algorithm on the mean multi-view depth fitting error.}
    \label{fig:quan greedy}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures_supp/quan_ablation_kf_selection.jpg}
    \caption{Reconstructed invisible details and visualization of per-vertex errors in several frames. From top to bottom are results with both energies, without the pose energy and without the visibility energy, respectively.}
    \label{fig: supp quantitative ablation study kf selection}
    \vspace{-0.4cm}
\end{figure}

\section{Additional Experiments}

\noindent\textbf{Intermediate Results}
In Fig.~\ref{fig:intermediate results}, given one current frame and its keyframe set, we demonstrate all the intermediate results including the reference color image, warped SMPL, dense reconstruction and color-encoded blending weights within the current frame and each keyframe.

%\noindent\textbf{More Quantitative Comparisons against DoubleFusion \cite{yu2018doublefusion} and PIFu \cite{saito2019pifu}}

\noindent\textbf{Quantitative Comparison against Greedy Algorithm} Fig.~\ref{fig:quan greedy} demonstrates the mean multi-view fitting errors of the results using the dynamic programming (DP) and greedy algorithm, respectively. And the average error of the whole sequence using DP and greedy algorithm are 0.7507 cm and 0.7732 cm, respectively. It shows that dynamic programming can produce the global optimum by considering the energy sum of the whole sequence, and achieve more physically accurate reconstruction.

\noindent\textbf{Quantitative Ablation Study of Pose-guided Keyframe Selection} Besides the mean vertex errors demonstrated in the main paper (Fig.~{\color{red}13})
%\ref{fig:quantitative ablation study kf selection}
, we also show the reconstructed results and visualization of per-vertex errors in this ablation study in Fig.~\ref{fig: supp quantitative ablation study kf selection}. It shows that with both visibility and pose guidance, the selected keyframe can cover invisible regions and share the similar poses with the current frame, so that physically plausible invisible details are recovered.





%\noindent\textbf{Evaluation of Adaptive Blending Weight}
%We evaluate the proposed adaptive blending weight (Eq.~\ref{eq: blending weight}) with the uniform weight both qualitatively and quantitatively in Fig.~\ref{fig:eval blending weight}. Fig.~\ref{fig:eval blending weight}(b) shows that the uniform blending weight oversmooths the geometric surface and even loses some body parts. We further evaluate the mean multi-view depth fitting errors using the two weights respectively in Fig.~\ref{fig:eval blending weight}(c), and it shows that the adaptive blending weight reconstructs much more accurate geometry because it attenuates the influence of incorrect inference and preserves more surface details.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{figures/eval_blending_weight.png}
%    \caption{Evaluation of the adaptive blending weight. (a)(b) Reconstructed results using the adaptive and uniform blending weights respectively, (c) mean multi-view depth fitting errors using the two blending weights respectively.}
%    \label{fig:eval blending weight}
%    \vspace{-0.4cm}
%\end{figure}



